Continuity-Discrimination Convolutional Neural Network for Visual Object Tracking

This paper proposes a novel model, named Continuity-Discrimination Convolutional Neural Network (CD-CNN), for visual object tracking. Existing state-of-the-art tracking methods do not deal with temporal relationship in video sequences, which leads to imperfect feature representations. To address this problem, CD-CNN models temporal appearance continuity based on the idea of temporal slowness. Mathematically, we prove that, by introducing temporal appearance continuity into tracking, the upper bound of target appearance representation error can be sufficiently small with high probability. Further, in order to alleviate inaccurate target localization and drifting, we propose a novel notion, object-centroid, to characterize not only objectness but also the relative position of the target within a given patch. Both temporal appearance continuity and object-centroid are jointly learned during offline training and then transferred for online tracking. We evaluate our tracker through extensive experiments on two challenging benchmarks and show its competitive tracking performance compared with state-of-the-art trackers.

==> 2_related_work.tex <==
\section{Related Work}
\label{sec:related_work}
\noindent {\bf Temporal slowness.} %As a possible learning principle for the emergence of receptive fields of complex cells in primary visual cortex (V1), %temporal slowness is based on the observation that the environment around us changes usually on a relatively slow time scale and thus the hypothesis that so %should its internal representation.
As mentioned above, temporal slowness is possibly a learning principle for the emergence of receptive fields of complex cells in primary visual cortex.
Slowly varying features extracted from even the quickly varying signals can possibly reflect the inherent properties of the environment and thus are robust to frequently intensive transformations. %Moreover, innately receptive to coherent visual streams, our visual system performs amazingly at recognizing objects in %images. These phenomena naturally leads to the unsupervised temporal slowness learning of visual features.
In cognitive science and computer vision areas, various related researches have been carried out lately. Berkes \etal \citep{cogprints2804} presented the temporal slowness problem and investigated it as a learning principle for receptive fields using slow feature analysis.
%They design a new algorithm that determines a functions through which slowly varying signals can be extracted and their experimental results show that a single %unsupervised learning principle is accountable for a rich repertoire of receptive field properties, such as direction selectivity, non-orthogonal inhibition, %end-inhibition and side-inhibition.
Li \etal \citep{li_unsupervised_2008} reported that unsupervised temporal slowness learning %reflects a certain recognitive mechanism that
enables the responses of neurons to be selective to different objects, yet tolerant or invariant to changes in object position, scale and pose.
Zou \etal \citep{Zou2012DeepLO} proposed %takes an alternative of training a hierarchical network for image classification. Taking tracked sequences as input,
a hierarchical network to learn invariant features with a temporal slowness constraint. The resulting spatial feature representation is well suited for the still image classification problem. For visual object tracking, temporal slowness remains unexplored. However, we will show in this paper that this principle is essential and can be transferred to help boost the performance of state-of-the-art trackers.

\noindent {\bf Objectness in tracking.} Objectness can serve as an important discriminator for object tracking. Wang \etal \citep{wang2015transferring} introduced objectness by offline pre-training a CNN to learn generic object features which distinguish objects against background. The output of the CNN is a $50 \times 50$ probability map for objectness. %with each indicating the probability that the corresponding input region belongs to an object.
%However, its objectness pre-training does not take into account positional centroid (that is, the relative position of target against the patch) in a straightforward way and therefore
An exhaustive online search is required for bounding box determination at each frame based on extra parameters.
Furthermore, the mapping from the objectness probability map into the raw image %introduces more artificial effect and
may cause inaccurate target localization especially in face of occlusion and background clutter.
In contrast, we propose object-centroid learning to jointly model objectness and positional centroid of the target within a given patch directly. Consequently, object-centroid endows our network with discriminative sensitivity to objectness with proper centroid.

%\noindent {\bf Deep learning models.} %Feature extraction and representation is of great significance to computer vision. Apparently,
%Deep features have shown their superior advantages over conventional handcrafted ones ever since Krizhevsky \etal proposed AlexNet \cite{NIPS2012_4824}. %with its significantly improved image classification performance in ImageNet challenge \cite{ILSVRC15}.
%Many other powerful feature extractors, such as GoogleNet\cite{szegedy2015going}, VGG Net\cite{simonyan2014very}, ResNet\cite{DBLP:journals/corr/HeZRS15}, were then invented and widely applied to computer vision tasks. However, feature extraction from these deep CNNs designed for classification tasks might not be well-suited for visual tracking because high-level features are inherently lack of high spatial resolutions for precise target localization.
%%in spite of the richness of category-level semantics.
%In this paper, PVANET is adopted as the backend of our model. With high computational efficiency and proper tradeoff between spatial resolution and semantics, PVANET is more appropriate for continuity and object-centroid learning.


==> 5_analysis.tex <==
\section{Analysis}
In this section, we present the upper bound of target prediction error by our tracker and empirically analyze the effectiveness of the offline joint learning of appearance continuity and object-centroid discrimination.

\subsection{Target Prediction Error}
The target prediction error incurred by our tracking method can be defined as the Euclidean distance between the features of predicted and ground-truth targets: $\mathcal{E} = \sum_j{\sqrt{{(\hat{Loss}}_j)}}/m + n(\delta + K\Delta t)$, where $P_*^{(t)}$ is the ground-truth and ${\hat P}_*^{(t)}$ is the predicted target patch at $t$th frame.

\begin{thm}[Upper Bound of Target Prediction Error]
With probability larger than $1-\rho$, the target prediction error $\mathcal{E}$ is upper-bounded by $\sum_j{\sqrt{{(\hat{Loss}}_j)}}/m + n(\delta + K\Delta t)$, for any $\delta > \sqrt{{n \over m} max_i{Var\left(\Phi_i\right)}}$, where $\hat{Loss}_j$ is ??? with respect to positive sample $P_j^{(t)}$ and $\rho = n\max_i{Var(\Phi_i)}/{m\delta^2}$.
\end{thm}

\iffalse
\begin{proof}
\begin{equation}
\begin{split}
error
& = {\left\lVert \Phi\left({\hat P}_*^{(t+1)}\right)-\Phi\left(P_*^{(t+1)}\right) \right\rVert}_2 \\
& = {\left\lVert \Phi\left({\hat P}_*^{(t+1)}\right)-\Phi\left(P_*^{(t)}\right)+\Phi\left(P_*^{(t)}\right)-\Phi\left(P_*^{(t+1)}\right) \right\rVert}_2 \\
& \le {\left\lVert \Phi\left({\hat P}_*^{(t+1)}\right)-\Phi\left(P_*^{(t)}\right) \right\rVert}_2 + \epsilon \\
& = {\left\lVert \Phi\left({\hat P}_*^{(t+1)}\right)-\frac{1}{m}\displaystyle\sum_{j=1}^m\Phi\left(P_j^{(t)}\right)+\frac{1}{m}\displaystyle\sum_{j=1}^m\Phi\left(P_j^{(t)}\right)-\Phi\left(P_*^{(t)}\right) \right\rVert}_2 + \epsilon \\
& \le {\left\lVert \Phi\left({\hat P}_*^{(t+1)}\right)-\frac{1}{m}\displaystyle\sum_{j=1}^m\Phi\left(P_j^{(t)}\right) \right\rVert}_2 +  {\left\lVert \frac{1}{m}\displaystyle\sum_{j=1}^m\Phi\left(P_j^{(t)}\right)-\Phi\left(P_*^{(t)}\right) \right\rVert}_2 + \epsilon \\
& = {\left\lVert \Phi\left({\hat P}_*^{(t+1)}\right)-\frac{1}{m}\displaystyle\sum_{j=1}^m\Phi\left(P_j^{(t)}\right) \right\rVert}_2 + {\left\lVert \overline{\Phi\left(P^{(t)}\right)} - \Phi\left(P_*^{(t)}\right) \right\rVert}_2 + \epsilon \\
& \le {\left\lVert \Phi\left({\hat P}_*^{(t+1)}\right)-\frac{1}{m}\displaystyle\sum_{j=1}^m\Phi\left(P_j^{(t)}\right) \right\rVert}_2 + {\left\lVert \overline{\Phi\left(P^{(t)}\right)} - \Phi\left(P_*^{(t)}\right) \right\rVert}_1 + \epsilon \\
& = {\left\lVert \Phi\left({\hat P}_*^{(t+1)}\right)-\frac{1}{m}\displaystyle\sum_{j=1}^m\Phi\left(P_j^{(t)}\right) \right\rVert}_2 + \displaystyle\sum_{i=1}^n{\left\vert \overline{\Phi_i\left(P^{(t)}\right)}-\Phi_i\left(P_*^{(t)}\right) \right\vert} + \epsilon
\end{split}
\end{equation}
where $P_j^{(t)}$ is the $j$th positive samples drawn around $P_*^{(t)}$ and $\overline{\Phi_i\left(P^{(t)}\right)}$ denotes the arithmetic mean. Mathematically, it is assumed that, in the $n$-dimensional feature space, the random vector, $\Phi$, conforms to some unknown distribution $\mathbb{P}(\varphi)$, whose expectation is given by
\begin{equation}
\mathbb{E}\left[\Phi\left(P_j^{(t)}\right)\right]=\int_{\varphi \in \mathfrak{R}^n} \varphi\, d\mathbb{P}(\varphi) =  \Phi\left(P_*^{(t)}\right)
\end{equation}
By Chebyshev inequality and Inclusion-exclusion Principle,
\begin{equation}
\begin{split}
\mathbb{P}\left(\bigcap_{i=1}^n {\left\vert \overline{\Phi_i\left(P^{(t)}\right)} - \Phi_i\left(P_*^{(t)}\right) \right\vert < \delta}\right)
& \ge 1 - \displaystyle\sum_{i=1}^n {\mathbb{P}\left(\left\vert \overline{\Phi_i\left(P^{(t)}\right)} - \Phi_i\left(P_*^{(t)}\right) \right\vert \ge \delta\right)} \\
& \ge 1 - \frac{1}{m\delta^2}\displaystyle\sum_{i=1}^n{Var(\Phi_i)} \\
& \ge 1 - \frac{n}{m\delta^2}\max_i{Var(\Phi_i)}
\end{split}
\end{equation}
Consequently, with the lower-bounded probability above, the prediction error occurred at each time slot is upperly-bounded by
\begin{equation}
\begin{split}
error
& \le {\left\lVert \Phi\left(\hat{P}_*^{(t+1)}\right) - \frac{1}{m}\displaystyle\sum_{j=1}^{m}{\Phi\left(P_j^{(t)}\right)} \right\rVert}_2 + \displaystyle\sum_{i=1}^{n}{\left\vert \overline{\Phi_i\left(P^{(t)}\right)} - \Phi_i\left(P_*^{(t)}\right)\right\vert} + {\epsilon} \\
& \le \frac{1}{m}\displaystyle\sum_j{\left\lVert \Phi\left(\hat{P}_*^{(t+1)}\right) - \Phi\left(P_j^{(t)}\right) \right\rVert}_2 + n\delta + \epsilon \\
& = {1 \over m} \displaystyle\sum_j{\sqrt{{\left\lVert \Phi\left(\hat{P}_*^{(t+1)}\right) - \Phi\left(P_j^{(t)}\right) \right\rVert}_2^2}}+n\delta+\epsilon \\
& \le \frac{1}{m}\displaystyle\sum_j{{\left(\hat{Loss_j}\right)}^{1 \over 2}} + n\left(\delta + C\Delta t\right)
\end{split}
\end{equation}
\end{proof}
\fi
\noindent The proof of Theorem 1 is presented in the supplemental material.
According to Theorem 1, for a tight upper bound, $\delta$ and $\Delta t$ should be $O\left({1 \over n^{1+\alpha}}\right)$, and thus, with a large probability, the number of samples drawn from each frame, $m=O\left(n^{3+\alpha}\right)$, for any small $\alpha>0$. This indicates that, with $O\left(n^{3+\alpha}\right)$ samples, the estimation error can be upperly-bounded by some small number with some large probability, if the generalisation loss $\hat{Loss}$ converges.

\iffalse
\begin{thm} [Object-centroid Learning Hardness]
The presence of $\mathcal{L}^\mathfrak{D}\left(P_j^{(t)}, N_l^{(t)}\right)$, in \eqref{eq:total_loss}, makes the discrimination learning much easier, suppose the generalisation loss $\hat{Loss}_{j,k,l} := \mathcal{L}^\mathfrak{C}\left({\hat P}_j^{(t)}, {\hat P}_k^{(t+1)}\right) + \left(\lambda \mathcal{L}^\mathfrak{D}+\mu \mathcal{L}^\mathfrak{S}\right) \left({\hat P}_j^{(t)}, {\hat N}_l^{(t)}\right)$ converges, where ${\hat P}_j^{(t)}$, ${\hat P}_k^{(t+1)}$ and ${\hat N}_l^{(t)}$ are all samples drawn during a testing phase.
\end{thm}
\fi

\iffalse
\begin{proof}
Suppose the generalisation loss converges, that is, there exists a small number, $\xi$, \st, for any ${\hat P}_j^{(t)}$, ${\hat P}_k^{(t+1)}$, ${\hat N}_l^{(t)}$,
\begin{equation}
\mathcal{L}^\mathfrak{C}\left({\hat P}_j^{(t)}, {\hat P}_k^{(t+1)}\right) + \left(\lambda \mathcal{L}^\mathfrak{D}+\mu \mathcal{L}^\mathfrak{S}\right) \left({\hat P}_j^{(t)}, {\hat N}_l^{(t)}\right) \le \xi
\end{equation}
then,
\begin{equation}
\begin{split}
\left\vert {\left\lVert \Phi\left({\hat P}_j^{(t)}\right)-\Phi\left({\hat P}_k^{(t)}\right) \right\rVert}_2 - \epsilon \right\vert
& \le {\left\lVert \Phi\left({\hat P}_j^{(t)}\right)-\Phi\left({\hat P}_k^{(t)}\right)-\Phi\left({\hat P}_k^{(t+1)}\right)+\Phi\left({\hat P}_k^{(t)}\right) \right\rVert}_2 \\
& = {\left\lVert \Phi\left({\hat P}_j^{(t)}\right)-\Phi\left({\hat P}_k^{(t+1)}\right) \right\rVert}_2 \le \sqrt\xi
\end{split}
\end{equation}
\begin{equation}
\epsilon-\sqrt\xi \le {\left\lVert \Phi\left({\hat P}_j^{(t)}\right)-\Phi\left({\hat P}_k^{(t)}\right) \right\rVert}_2 \le \epsilon+\sqrt\xi
\end{equation}
on the other hand,
\begin{equation}
\lambda \mathcal{L}^\mathfrak{D} \left({\hat P}_j^{(t)}, {\hat N}_l^{(t)}\right) = \lambda exp\left(-\beta{\left\lVert \Phi\left({\hat P}_j^{(t)}\right)-\Phi\left({\hat N}_l^{(t)}\right) \right\rVert}_2^2\right) \le \xi
%\forall P_j^{(t)}, N_l^{(t)},
\end{equation}
\begin{equation}
{\left\lVert \Phi\left({\hat P}_j^{(t)}\right)-\Phi\left({\hat N}_l^{(t)}\right) \right\rVert}_2 \ge \sqrt{{1 \over \beta}log{\lambda \over \xi}}
\end{equation}
Choose $c_0$ with $(\epsilon + \sqrt\xi)/2=\max_j{\left\lVert c_0 - \Phi\left({\hat P}_j^{(t)}\right) \right\rVert}_2$. We obtain, for any ${\hat N}_l^{(t)}$,
\begin{equation}
\begin{split}
{\left\lVert c_0 - \Phi\left({\hat N}_l^{(t)}\right) \right\rVert}_2
& \ge \left\vert {\left\lVert c_0 - \Phi\left({\hat P}_j^{(t)}\right) \right\rVert}_2 - {\left\lVert \Phi\left({\hat P}_j^{(t)}\right) - \Phi\left({\hat N}_l^{(t)}\right) \right\rVert}_2\right\vert \\
& = {\left\lVert \Phi\left({\hat P}_j^{(t)}\right) - \Phi\left({\hat N}_l^{(t)}\right) \right\rVert}_2 - {\left\lVert c_0 - \Phi\left({\hat P}_j^{(t)}\right) \right\rVert}_2 \\
& \ge \sqrt{{1 \over \beta}log{\lambda \over \xi}} - \frac{\epsilon + \sqrt\xi}{2}
\end{split}
\end{equation}
Therefore, any decision boundary of an analytical form ${\left\lVert x- c_0 \right\rVert}_2 = R(x)$ can separate positives and negatives, where $R: \mathfrak{R}^n \mapsto \mathfrak{R}$, \st $(\epsilon + \sqrt\xi)/2 < R(x) < \sqrt{{1 \over \beta}log{\lambda \over \xi}} - $(\epsilon + \sqrt\xi)/2$. This indicates that the presence of $\mathcal{L}^\mathfrak{D}\left(P_j^{(t)}, N_l^{(t)}\right)$, in \eqref{eq:total_loss} can yield a large gap in the Hilbert space. And the decision boundary with such a gap can be learned more easily by a two-layer MLP than without $\mathcal{L}^\mathfrak{D}\left(P_j^{(t)}, N_l^{(t)}\right)$.
\end{proof}
\fi

\subsection{Effectiveness of Offline Joint Learning}
To empirically validate the effectiveness of our formulation in offline joint learning, we implement and test several variations of CD-CNN. Specifically, we implement offline training without object-centroid distance loss $\mathcal{L}^\mathfrak{D}(\cdot, \cdot)$ for justifying its necessity. This variant model is denoted by CD-CNN-wo-Dloss. To verify the joint necessity of the appearance continuity loss and object-centroid distance loss, we implement offline training with explicit object-centroid discrimination learning only, denoted by CD-CNN-SlossOnly. To validate the object-centroid learning for generic objects, for each test sequence in online tracking, the fully-connected layers, fc3 and fc4, are finetuned from scratch without being initialized through object-generic offline training. This target-specific online finetuned model is denoted by CD-CNN-tarspec. Besides, we train the network using $\mathcal{L}^\mathfrak{P}(\cdot, \cdot)$ instead of $\mathcal{L}^\mathfrak{S}(\cdot, \cdot)$ with no other adjustment to verify the effectiveness of appearance continuity transferring. As illustrated in Figure \ref{fig:internal_comp:b}, all the variations above do not perform as well as our original CD-CNN, which validates appearance continuity transferring as well as object-centroid discrimination and the overall loss formulation of \eqref{eq:total_loss} in the offline joint learning.

\iffalse
\begin{figure}[t]
	\centering
	\begin{varwidth}[t]{\textwidth}
		\includegraphics[width=0.45\linewidth]{internal_comp_precision.eps}
	\end{varwidth}
	\qquad
	\begin{varwidth}[t]{\textwidth}
		\includegraphics[width=0.45\linewidth]{internal_comp_success.eps}
	\end{varwidth}
	\caption{Precision plots and success plots of OPE on the CVPR2013 Benchmark for the internal comparisons.}
	\label{fig:internal_comp}
\end{figure}
\fi 
